VSS Challenge Problem: Verifying the Correctness of AllReduce Algorithms in the MPICH Implementation of MPI

We describe a challenge problem for verification based on the MPICH implementation of MPI. The MPICH implementation includes several algorithms for allreduce, all of which should be functionally equivalent to reduce followed by broadcast. We created standalone versions of three algorithms and verified two of them using CIVL.

==> eptcsdata.tex <==
\providecommand{\firstpage}{90}
\providecommand{\publicationstatus}{S.F.\ Siegel and G.\ Gopalakrishnan (Eds.):\\
International Workshop on Verification of\\
Scientific Software (VSS 2025)\\
EPTCS 432, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.432.10}{10.4204/EPTCS.432.10}}
\pdfoutput=1

